Projection Regret: Reducing Background Bias for Novelty Detection via Diffusion Models

Novelty detection is a fundamental task of machine learning which aims to detect abnormal ($\textit{i.e.}$ out-of-distribution (OOD)) samples. Since diffusion models have recently emerged as the de facto standard generative framework with surprising generation results, novelty detection via diffusion models has also gained much attention. Recent methods have mainly utilized the reconstruction property of in-distribution samples. However, they often suffer from detecting OOD samples that share similar background information to the in-distribution data. Based on our observation that diffusion models can \emph{project} any sample to an in-distribution sample with similar background information, we propose \emph{Projection Regret (PR)}, an efficient novelty detection method that mitigates the bias of non-semantic information. To be specific, PR computes the perceptual distance between the test image and its diffusion-based projection to detect abnormality. Since the perceptual distance often fails to capture semantic changes when the background information is dominant, we cancel out the background bias by comparing it against recursive projections. Extensive experiments demonstrate that PR outperforms the prior art of generative-model-based novelty detection methods by a significant margin.

==> algorithm/Inner_Features.tex <==
\begin{algorithm}
\caption{Computation of input feature cosine distance}\label{alg:cosine_distance}
\begin{algorithmic}
\Require model $f_{\theta}$, data input $x$, cosine distance $cos$, noise timestep $t_{1}$, denoising timestep $t_{2}$, perturbation timestep $t_{3}$, projection ensemble $n_{1}$, evaluation ensemble $n_{2}$ 

\State Score $\gets 0$
\State $x_{\textit{feat}}$ \gets 
\For{$i= \left(1,...,n_{1} \right)$}
\State $x^{\prime} \gets x.clone()$
\State $z \gets \mathcal{N}(0,I)$
\State $x^{\prime} \gets f_{\theta}(x^{\prime}+\sigma_{t_{1}}z,t_{1})$ 
\For{$k = \left(1,...,n_{2} \right)$}
\State  $z_{k} \gets \mathcal{N}(0,I)$
\State Score $\mathrel{+}\mathrel{=}  d(f_{\theta}(x+\sigma_{t_{2}}z_{k},t_{2}),x) - d(f_{\theta}(x^{\prime}+\sigma_{t_{2}}z_{k},t_{2}),x^{\prime}) $
\EndFor
\EndFor \\
\Return $Score$
\end{algorithmic}
\end{algorithm}

==> algorithm/projection_regret.tex <==
\begin{algorithm}[t]
\caption{\textbf{Projection Regret} for out-of-distribution detection}\label{alg:main_algorithm}
\begin{algorithmic}
\Require Projection $\Pi_{\ptheta}^{t}$, data input $\rvx$, projection timesteps $\alpha$ and $\beta$, projection iterations $n_{\alpha}$ and $n_{\beta}$

\State $S_{\mathtt{PR}} \gets 0$
\For{$i= \left(1,...,n_{\alpha} \right)$}
\State $\rvz \gets \mathcal{N}(\mathbf{0},I)$
\State $\mathbf{x^{\prime}} \gets  \Pi_{\ptheta}^{t_{\alpha}}(\rvx,\rvz)$ 
\For{$k = \left(1,...,n_{\beta} \right)$}
\State  $\rvz_{k} \gets \mathcal{N}(\mathbf{0},I)$
\State $S_\mathtt{PR}$ $\gets S_\mathtt{PR}\mathrel{+} \text{LPIPS}(\Pi_{\ptheta}^{t_{\beta}}(\rvx,\rvz_{k}),\rvx) - \text{LPIPS}(\Pi_{\ptheta}^{t_{\beta}}(\mathbf{x^{\prime}},\rvz_{k}),\mathbf{x^{\prime}}) $
\EndFor
\EndFor \\
\Return $S_\mathtt{PR}$
\end{algorithmic}

\end{algorithm}

==> fig/fig_corruption.tex <==
\begin{figure}[t!]
    \centering
    \begin{subfigure}[c]{0.15\textwidth}
        \includegraphics[width=\textwidth]{fig/originalcifar10.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[c]{0.15\textwidth}
        \includegraphics[width=\textwidth]{fig/shotnoise.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[c]{0.15\textwidth}

        \includegraphics[width=\textwidth]{fig/defocusblur.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[c]{0.15\textwidth}
        \includegraphics[width=\textwidth]{fig/fog.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[c]{0.15\textwidth}
        \includegraphics[width=\textwidth]{fig/elastic.png}
    \end{subfigure}
    \caption{\textbf{Different types of corruption.} Original CIFAR-10 data and its corruption. From left, original data, shot noise, defocus blur, fog, and elastic transform. The corruption level is 3. }
    \label{fig:corruption}
\end{figure}


==> fig/fig_visual_analysis.tex <==
\begin{figure}[t]
	\begin{center}
		\centerline{\includegraphics[width = 0.6\columnwidth]{fig/LPIPS_analysis.png} }
 
    
		\vskip -0.15in
	\end{center}
		\vskip -0.15in
	   \caption{ \textbf{Visual analysis of OOD samples.} \textbf{(a):} CIFAR-100 samples that show smallest uncertainty in the $S_{\mathtt{proj},\mathtt{LPIPS}}$ metric in Table \ref{table:ablate}. Image with limited background information is favored. \textbf{(b):} Their projections through consistency models. 
    }
    \label{fig:visual_analysis}
\end{figure}

==> fig/figure_sensitivity.tex <==
\begin{figure}[t!]
    \centering
    \begin{subfigure}[c]{0.17\textwidth}

        \includegraphics[width=\textwidth]{fig/heatmap_svhn.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[c]{0.17\textwidth}
        \includegraphics[width=\textwidth]{fig/heatmap_lsun.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[c]{0.17\textwidth}
        \includegraphics[width=\textwidth]{fig/heatmap_imgn.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[c]{0.23\textwidth}
        \includegraphics[width=\textwidth]{fig/cifar10lsun.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[c]{0.23\textwidth}
        \includegraphics[width=\textwidth]{fig/cifar10imgn.pdf}
    \end{subfigure}
    \caption{\textbf{Sensitivity analysis on \methodname.} Left three replicate Figure 4 in the SVHN \textbf{(left)}, LSUN \textbf{(middle)}, and ImageNet \textbf{(right)} datasets. Right two replicate Figure 3 in LSUN \textbf{(left)} and ImageNet \textbf{(right)} datasets. In-distribution is the CIFAR-10 dataset.}
    %\caption{\textbf{Sensitivity analysis of Figure 3 in other datasets.} We also experiment in LSUN \textbf{(left)} and ImageNet \textbf{(right)}.}
    \label{fig:sensitivity}

\end{figure}


==> method.tex <==
\section{Method}
\label{section:method}

%첫 번째 파트: DIffusion model의 문제를 NOIse-level별로 본다면 noise level이 작을 때에는 ood 또한 잘 reconstruct되면 noise level이 높을 시 output이 blurry하다. 하지만 consistency-model은 one-shot generation이 쉽게 가능하다는 장점ㅁ이 있다. 우리는 먼저 consistency model에서 data와 이의 reconstruction간의 LPIPS distance metric이 challenging한 CIFAR-100 dataset에서 OOD detection 성능을 기존 method에 비해 높일 수 있다는 것을 보여준다.


%우리의 hypothesis: ID를 consistency model에 넣고 돌렸을 때 reconstruct된 새로운 ID data와 original data 간의 Perceptual distance가 OOD를 consistency model에 넣고 돌렸을 때 reconstruct된 새로운 ID data와 original OOD data 간의 perceptual distance보다 여러 noise에 대해서 평균했을 때 더 작다.


%여기 섹션에서는 projection regret에 대해 설명할 것입니다. LPIPS metric이 꽤 좋은 성능을 보였지만 여전히 LPIPS 정보는 배경을 가지고 동작할 수 있습니다. 그에 대한 증거로 appendix에 minimum LPIPS를 보이는 OOD CIFAR-100  data가 단순한 data를 가지고 있다는 걸 보여줄 것입니다. 그렇기 때문에 우리는 Consistency modeld을 이용해서 Input data를 그와 similar한 background를 가진 ID로 보내고 r각각에서 Motivation section에서 설명한 LPIPS metric을 구할 것입니다. 최종적인 metric은 둘 간의 차이입니다. 
\input{fig/fig_why_use_lpips}
\input{fig/fig_AUROC_cm_edm}
\input{algorithm/projection_regret}

\subsection{Utilizing projection for OOD detection.}
\label{section:method:projection}

In this section, we first analyze the traits of in-distribution and out-of-distribution images and their projection. Specifically, given an input image $\rvx$ and time index $i$ defined in Section \ref{section:pre:diff}, we sample a projection output from the projection distribution $\Pi_{\ptheta}^{t_{i}}(\rvx)$ by sampling a random noise $\rvz \sim \mathcal{N}(\bm{0},\mathbf{I})$ and computing $\Pi_{\ptheta}^{t_{i}}(\rvx,\rvz)$. 

Figure \ref{fig:oods_andprojections} shows the projection evaluated on the CIFAR-100 \citep{Krizhevsky09} and SVHN \citep{Netzer11} OOD images evaluated in the pre-trained CIFAR-10 consistency model with $i=8$ $(t_{i}=1.92)$. We can see semantic changes in images while background statistics have not changed much. Furthermore, when evaluated in the in-distribution CIFAR-10 dataset, the shift is not as drastic as in the OOD dataset.

Since the commonly used $\ell_{2}$ distance does not differentiate the background and semantic statistics, we instead propose to use perceptual distance as the OOD detection metric. We use LPIPS \citep{Zhang18} evaluated in the vgg backbone \citep{Simonyan14} as the perceptual distance since it is used to measure reconstruction quality in various vision-based tasks \citep{Ma20sup, Whang22blur}. For verification, we first define the averaged distance between the input image $\rvx$ and the projection distribution $\Pi_{\ptheta}^{t}(\rvx)$ expressed as follows.
\begin{align}
    S_{\mathtt{\Pi}}^{d}(\rvx,t)= \mathbb{E}_{\rvz \sim \mathcal{N}(\bm{0},\mathbf{I})} d(\rvx, \Pi_{\ptheta}^{t}(\rvx,\rvz)) 
\end{align}
where $d$ is the distance metric. We propose $ S_{\mathtt{\Pi}}^{\text{LPIPS}}(\rvx,t)$ as our base metric
and compare its performance against $S_{\mathtt{\Pi}}^{\ell_{2}}$ that use the $\ell_{2}$ distance. Furthermore, we also compare the method that uses the averaged LPIPS and $\ell_{2}$ distance between the input image and its imperfect projection distribution $\pi_{\ptheta}^{t}$ evaluated on the edm diffusion model \citep{Karras22} instead of the projection and denote them as $S_{\mathtt{\pi}}^{\text{LPIPS}}$ and $S_{\mathtt{\pi}}^{\ell_{2}}$, respectively. For all methods, we perform sampling on 100 random noises $\rvz$.

We report the AUROC on the CIFAR-10 vs (CIFAR-100, SVHN) task in Figure \ref{fig:quantitative_analysis}. Our proposed metric, $S_{\mathtt{\Pi}}^{\text{LPIPS}}$ shows the best performance and even exceeds the performance of existing diffusion-model-based OOD detection methods in the CIFAR-10 vs CIFAR-100 task. On the other hand, $\ell_{2}$ distance as a metric outputs a lower distance in the SVHN OOD dataset than the CIFAR-10 in-distribution dataset. Finally, the best result is observed in the intermediate time step with a time index of $i=7$ and $i=8$. %since smaller noise will enable the reconstruction of OOD data and larger noise will change the semantics of the ID data either. We will discuss this further in the Appendix.


\subsection{\methodname}
\label{section:method:projectionregret}

While the perceptual distance performs better than the $\ell_{2}$ distance, they may fail to capture the semantic change when background information is dominant. For example, we refer to Figure \ref{fig:method:method} for the failure case of $S_{\mathtt{\Pi}}^{\text{LPIPS}}$. While the projection of the OOD (bridge) shows in-distribution (church) semantics, the area of the changed region is relatively small, and thereby $S_{\mathtt{\Pi}}^{\text{LPIPS}}$ outputs a lower abnormality score on OOD data than the in-distribution data.

We propose our algorithm, \methodname to reduce the background bias further. We show the full computation procedure in Algorithm \ref{alg:main_algorithm} and Figure \ref{fig:method:method}. Based on our observation in Section \ref{section:method:projection}, we first project the input image $\rvx$ by the given time index $\alpha$ and standard white noise $\rvz\sim \mathcal{N}(\bm{0},\mathbf{I})$.
\begin{align}
    \mathbf{x^{\prime}}=\Pi_{\ptheta}^{t_{\alpha}}(\rvx,\rvz)
\end{align}
For the input image $\rvx$ and projected image $\mathbf{x^{\prime}}$, we again compute $S_{\mathtt{\Pi}}^{\text{LPIPS}}$ proposed in Section \ref{section:method:projection}. Since we regard the background bias to be similar in the input image $\rvx$ and the projected image $\mathbf{x^{\prime}}$, we output the difference between the two to compute our metric $S_{\mathtt{PR}}$ as follows. 

\begin{align}
    S_{\mathtt{PR}}(\rvx,\alpha,\beta) = S_{\mathtt{\Pi}}^{\text{LPIPS}}(\rvx,t_{\beta}) -  \mathbb{E}_{\rvz \sim \mathcal{N}(\bm{0},\mathbf{I})} S_{\mathtt{\Pi}}^{\text{LPIPS}}(\Pi_{\ptheta}^{t_{\alpha}}(\rvx,\rvz),t_{\beta})
\end{align}

Furthermore, to alleviate the variance on the random noise, we sample $\rvz$ by $n_{1}$ times to generate the mapped image and sample the random noise for $n_{2}$ times to compute the distance metric $S_{\mathtt{\Pi}}^{\text{LPIPS}}$ for each input image and its projection.

Finally, selection for the time index hyperparameter is always a burden for the practical use of the OOD detection model since we do not know the OOD information in advance. Furthermore, the best hyperparameter may vary across the type of OOD. Therefore, we also propose an ensemble approach that outputs the sum of distance calculated in different time index hyperparameter setups. We discuss the effect of each component in Section \ref{section:exp:experiment-analysis}.

==> motivation.tex <==
\input{table/table_motivation}

\section{Motivation}
\label{section:motivation}

\subsection{Projection}
We first define projection that is shown in Figure \ref{fig:method:proj}. We define projection $\Pi_{\ptheta}^{t}(\rvx,\rvz)$ as a final output $\rvx_{0}$ of the reverse-time SDE that is initialized from the noised image $\rvx+t\rvz$ in time $t$. This can be achieved deterministically by multi-step sampling via the ODE-solvers of the diffusion models or the 1-step output of the consistency model. Furthermore, we define a projection distribution of input image $\rvx$ in time $t$ as $\Pi_{\ptheta}^{t}(\mathbf{x^{\prime}} \mid \rvx) \coloneqq \Pi_{\ptheta}^{t}(\rvx,\rvz)$ where $\rvz \sim \mathcal{N}(\bm{0},\mathbf{I})$ . This corresponds to the distribution of achievable projections on time $t$ given input image $\rvx$. We abbreviate $\Pi_{\ptheta}^{t}(\mathbf{x^{\prime}}\mid \rvx)$ as
$\Pi_{\ptheta}^{t}(\rvx)$.

We also define imperfect projection $\pi_{\ptheta}^{t}(\rvx,\rvz)=D_{\ptheta}(\rvx + t\rvz,t)$ as the one-step output of the diffusion model initialized from the same image $\rvx+t\rvz$ and time $t$ and $\pi_{\ptheta}^{t}(\rvx)$ respectively.

\subsection{Motivation}
This section analyzes the pitfalls of existing diffusion-model-based OOD detection methods. Primarily, we hypothesize that background statistics dominate such methods' metrics and hence the existing methods struggle on detecting OOD with similar backgrounds but different semantics. 

We validate our hypothesis by testing MSMA \citep{Mahmood21} as a baseline method. MSMA uses the $\ell_{2}$ norm of the score function as the metric, where the score function is $\ell_{2}$ distance between the input image $\rvx$ and imperfect projection of the diffusion model $\pi_{\ptheta}^{t}(\rvx,\rvz)$.
\begin{align}
    S_{\mathtt{MSMA}}(\rvx,t) = \mathbb{E}_{\rvz \sim \mathcal{N}(\bm{0},\mathbf{I})} \| \frac{ \pi_{\ptheta}^{t}(\rvx,\rvz)-\rvx}{t} \|_{2}^{2}
\end{align}
Then, they ensemble this metric across multiple time steps to construct a normality vector. Furthermore, they train a one-class classifier over the training data's normality vector and use the classifier's confidence metric to compute the abnormality score.

We evaluate MSMA trained in CIFAR-10 on two OOD datasets: CIFAR-100 and rotated CIFAR-10 image dataset. These two datasets share similar backgrounds with CIFAR-10 dataset but show different semantics \citep{Gidaris18}. We report the result in Table \ref{table:motivation}. MSMA struggles on both datasets and especially almost fails to detect rotated CIFAR-10 datasets with an AUROC of 0.507. 

 We also test MSMA's performance on the resized LSUN \citep{Yu15} and the LSUN (FIX) \citep{Tack20} dataset, which is the smoothed LSUN dataset with reduced background noise. While the two dataset share similar semantics, the performance of MSMA drops from 0.956 to 0.547. We further provide visualization of LSUN and LSUN (FIX) dataset in Appendix.



==> table/table_lsun.tex <==
\begin{table}[t!]
\centering
\caption{\textbf{OOD detection results (TNR at 95\% TPR, AUROC) in LSUN.} Experiment is conducted in the LSUN dataset with bedroom as in-distribution. OOD datasets are bridge/church/classroom.} 
\label{table:lsun}
\small
%\resizebox{\textwidth}{!}{

\begin{tabular}{cccc}
\toprule   
Method & bridge & church & classroom\\ \midrule
LMD \citep{Liu23} & 0.033/0.386 & 0.060/0.379 & 0.007/0.336\\
\methodname & 0.443/0.830 & 0.253/0.772 & 0.120/0.696\\ 
\bottomrule
\end{tabular}
%}
\vskip -0.1in
\end{table}

==> table/table_metrics.tex <==
\begin{table}[t!]
\centering
\caption{\textbf{Results with different OOD detection metrics.} In-distribution dataset is the CIFAR-10 dataset. We report AUROC, TNR at 95\% TPR, detection accuracy, AUPR\_IN, and AUPR\_OUT. Higher is better in all metrics.}
\label{table:metric}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lllll}
\toprule   
Method & SVHN & CIFAR-100 & LSUN& ImageNet \\\midrule
LMD \citep{Liu23} & 0.979/0.890/0.924/0.955/0.992 & 0.620/0.112/0.591/0.602/0.612 & 0.734/0.206/0.678/0.722/0.721 & 0.686/0.168/0.637/0.674/0.677 \\ 
\methodname & 0.993/0.967/0.961/0.982/0.997 & 0.775/0.283/0.703/0.768/0.771 & 0.836/0.313/0.761/0.849/0.808 & 0.813/0.326/0.736/0.818/0.804 \\ 
\bottomrule
\end{tabular}}
\vskip -0.1in
\end{table}

==> table/table_motivation.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Performance (AUROC) of MSMA \citep{Mahmood21} on proposed OOD datasets.}}
\label{table:motivation}
\scalebox{0.85}{%
\begin{tabular}{ccccc}
\toprule
Method & CIFAR100 & Rotated CIFAR-10 & LSUN & LSUN (FIX)\\\midrule
MSMA & 0.579 & 0.507 & 0.945 & 0.587\\
\bottomrule
\end{tabular}}
\end{table}

==> table/table_robustness.tex <==
\begin{table}[t!]
\centering
\caption{\textbf{OOD detection results (AUROC) under the corrupted in-distribution data.} In-distribution dataset is CIFAR-10 and OOD datasets are SVHN/CIFAR-100/LSUN/ImageNet. We denote level 0 as the performance of \methodname in uncorrupted in-distribution dataset.}
\label{table:robustness}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccc}
\toprule   
Noise type & level 0 & level 1 & level 2 & level 3\\\midrule
Shot noise & 0.993/0.775/0.836/0.813 & 0.972/0.641/0.700/0.682 & 0.936/0.526/0.577/0.566 & 0.811/0.310/0.336/0.339\\
Defocus blur & 0.993/0.775/0.836/0.813 & 0.992/0.760/0.822/0.800 & 0.990/0.723/0.790/0.766 & 0.986/0.666/0.735/0.711\\
Fog & 0.993/0.775/0.836/0.813 & 0.989/0.701/0.769/0.745 & 0.980/0.570/0.641/0.620 & 0.969/0.480/0.543/0.529 \\
%Snow & 0.993/0.775/0.836/0.813 & 0.990/0.723/0.791/0.766 & 0.960/0.541/0.600/0.585 & 0.975/0.606/0.673/0.652\\
Elastic & 0.993/0.775/0.836/0.813 & 0.989/0.693/0.763/0.738 & 0.989/0.692/0.762/0.737 & 0.987/0.659/0.731/0.706 \\

%Contrast & 0.993/0.775/0.836/0.813 & 0.987/0.674/0.743/0.720 & 0.963/0.466/0.523/0.513 & 0.939/0.353/0.391/0.394\\
\bottomrule
\end{tabular}}
\vskip -0.1in
\end{table}
